High-z gamma-ray burst detection by SVOM/ECLAIRs: Impact of instrumental biases on the bursts' measured properties

Context. Gamma-ray bursts (GRBs) can be detected at cosmological distances and therefore can be used to study the contents and phases of the early Universe. The 4-150 keV wide-field trigger camera ECLAIRs to fly on board the Space-based multi-band Variable Object Monitor (SVOM) mission, dedicated to studying the high-energy transient sky in synergy with multi-messenger follow-up instruments, has been adapted to detect high-redshift (high-z) GRBs. Aims. Investigating the detection capabilities of ECLAIRs for high-z GRBs and estimating the impacts of instrumental biases in reconstructing some of the source measured properties, focusing on GRB duration biases as a function of redshift. Methods. We simulated realistic detection scenarios for a sample of 162 already observed GRBs with known redshift values as they would have been seen by ECLAIRs. We simulated them at redshift values equal and higher than their measured value. Then, we assessed whether they would be detected with a trigger algorithm resembling that on board of ECLAIRs, and derived quantities such as T90, for those that would have been detected. Results. We find that ECLAIRs would be capable of detecting GRBs up to very high redshift values (e.g. 20 GRBs in our sample are detectable within more than 0.4 of the ECLAIRs field of view for z > 12). The ECLAIRs low-energy threshold of 4 keV, contributes to this great detection capability, as it may enhance it at high redshift (z > 10) by over 10% compared to a 15 keV low-energy threshold. We also show that the detection of GRBs at high-z values may imprint tip-of-the-iceberg biases on the GRB duration measurements, which can affect the reconstruction of other source properties.

==> acronyms.tex <==
% ----------- A -------------

% ----------- B -------------
\newacronym{bat}{BAT}{Burst Alert Telescope}
\newacronym{batse}{BATSE}{The Burst and Transient Source Experiment}
\newacronym{bh}{BH}{Black Hole}
% ----------- C -------------
\newacronym{catbat}{CatBAT}{$3^{rd}$ \textit{Swift} BAT Gamma--Ray Burst Catalogue}
\newacronym{catgbm}{CatGBM}{The Fourth \textit{Fermi}--GBM Gamma--Ray Burst Catalogue}
\newacronym{cgro}{\textit{CGRO}}{Compton Gamma-Ray Observatory}
\newacronym{cnes}{CNES}{Centre National d'études spatiales}
\newacronym{cnsa}{CNSA}{China National Space Administration}
\newacronym{cpl}{CPL}{Cut-Off Power Law}
\newacronym{cxb}{CXB}{Cosmic X-ray Background}
\newacronym{csnr}{cSNR}{count SNR}
%\newacronym{csnr}{cSNR}{count \gls{snr}}
% ----------- D -------------
%\newacronym{dec}{Dec}{Declination}
% ----------- E -------------
\newacronym{ecpi}{ECPI}{ECLAIRs general program Pipeline}

% ----------- F -------------
\newacronym{fcfov}{fcFoV}{fully-coded \gls{fov}}
\newacronym{fits}{FITS}{Flexible Image Transport System}
\newacronym{fov}{FoV}{Field of View}

% ----------- G -------------
\newacronym{gbm}{GBM}{Gamma-ray Burst Monitor}
\newacronym{gcn}{GCN}{Gamma-ray Coordinates Network}
\newacronym{gft}{GFT}{Ground Follow-up Telescope}

\newacronym{grb}{GRB}{Gamma Ray Burst}
\newacronym{grm}{GRM}{Gamma Ray burst Monitor}
% ----------- H -------------
% ----------- I -------------
\newacronym{icrs}{ICRS}{International Celestial Reference System}
%\newacronym{isnr}{iSNR}{image \gls{snr}}
\newacronym{isnr}{iSNR}{image SNR}



% ----------- J -------------

% ----------- K -------------

% ----------- L -------------
%\newacronym{lat}{LAT}{\textit{Large Area Telescope}}
\newacronym{lgrb}{LGRB}{Long Gamma-Ray Burst}
%\newacronym{leo}{LEO}{Low Earth Orbit}
\newacronym{lsst}{LSST}{\textit{Large Synoptic Survery Telescope}}
%\newacronym{lofar}{LOFAR}{\textit{Low-Frequency Array for radio astronomy}}


% ----------- M -------------

\newacronym{mxt}{MXT}{Microchannel X-ray Telescope}

% ----------- N -------------
\newacronym{ns}{NS}{Neutron Star}
% ----------- O -------------

% ----------- P -------------
\newacronym{pcfov}{pcFoV}{partially-coded \acrlong{fov}}
\newacronym{pira}{PIRA}{Particle Interactions Recycling Approach}
\newacronym{pl}{PL}{Power Law}


% ----------- Q -------------

% ----------- R -------------
%\newacronym{ra}{RA}{Right Ascension}

% ----------- S -------------
\newacronym{sbpl}{SBPL}{Smoothly Broken Power Law}
%\newacronym{saa}{SAA}{South Atlantic Anomaly}
%\newacronym{ska}{SKA}{\textit{Square Kilometre Array}}

\newacronym{sfr}{SFR}{Star Formation Rate}
\newacronym{sgrb}{SGRB}{Short Gamma-Ray Burst}

\newacronym{snr}{SNR}{Signal to Noise Ratio}
\newacronym{svom}{\textit{SVOM}}{\textit{Space-based multi-band Variable Object Monitor}}

% ----------- T -------------
\newacronym{ti}{TI}{time-integrated}
\newacronym{tr}{TR}{time-resolved}

% ----------- U -------------

% ----------- V -------------
\newacronym{vhf}{VHF}{Very High Frequency}
%\newacronym{vlt}{VLT}{\textit{Very Large Telescope}}
\newacronym{vt}{VT}{Visible Telescope}

% ----------- W -------------
% ----------- X -------------
%\newacronym{xrt}{XRT}{\textit{X-ray Telescope}}
% ----------- Y -------------

% ----------- Z -------------




